Contrast, Stylize and Adapt: Unsupervised Contrastive Learning Framework for Domain Adaptive Semantic Segmentation

To overcome the domain gap between synthetic and real-world datasets, unsupervised domain adaptation methods have been proposed for semantic segmentation. Majority of the previous approaches have attempted to reduce the gap either at the pixel or feature level, disregarding the fact that the two components interact positively. To address this, we present CONtrastive FEaTure and pIxel alignment (CONFETI) for bridging the domain gap at both the pixel and feature levels using a unique contrastive formulation. We introduce well-estimated prototypes by including category-wise cross-domain information to link the two alignments: the pixel-level alignment is achieved using the jointly trained style transfer module with the prototypical semantic consistency, while the feature-level alignment is enforced to cross-domain features with the \textbf{pixel-to-prototype contrast}. Our extensive experiments demonstrate that our method outperforms existing state-of-the-art methods using DeepLabV2. Our code is available at https://github.com/cxa9264/CONFETI

==> contents/tables/consistency.tex <==
\begin{table}[]
\centering
\small
\caption{Impact of the semantic consistency loss on the GTA $\rightarrow$ Cityscapes benchmark. }
\label{tab:abla_sem}
%\resizebox{\columnwidth}{!}{%

\begin{tabular}{ccccc}
\toprule
 & w/o $\mathcal{L}_\text{SC}$  & $\mathcal{L}_\text{CE}$  & MSE        & $\mathcal{L}_\text{SC}$  \\ 
 \midrule
 mIoU  & 58.0  & 58.6  & 61.6  & \textbf{62.2} \\ 
 \bottomrule
\end{tabular}%}
\end{table}

==> contents/tables/gta2cs_poster.tex <==
\begin{table*}[h]
\centering
\small
\caption{Comparison results on \textbf{GTA5 $\rightarrow$ Cityscapes}. Methods based on \colorbox{SpringGreen}{pixel alignment} are highlighted with colors. $^\dag$ indicate methods trained at higher resolution.}
\label{tab:gtacs}
\begin{tabular}{@{}cc@{}}
\toprule
Methods & mIoU \\ \midrule
DACS   & 52.1 \\
ProCA   & 56.3 \\
ProDA   & 57.5 \\
SePiCo  & 61.0 \\
\textbf{\method (Ours)} & \textbf{62.2} \\ \midrule
HRDA  $^\dag$ & 63.0 \\
\textbf{\method (Ours)}$^\dag$ & \textbf{63.3} \\ \bottomrule
\end{tabular}
\end{table*}

==> contents/tables/synthia2cs_poster.tex <==
\begin{table*}[h]
\centering
\small
\caption{Comparison results on \textbf{SYNTHIA $\rightarrow$ Cityscapes}.}
\label{tab:synthiacs}
\begin{tabular}{@{}c|cc@{}}
\toprule
Methods & mIoU & mIoU*  \\ \midrule
DACS   & 48.3 & 54.8  \\
ProCA   & 53.0 & 59.6  \\
ProDA   & 55.5 & 62.0  \\
SePiCo  & 58.1 & 66.5  \\
\textbf{\method (Ours)} & \textbf{58.7} & \textbf{67.4}  \\ \bottomrule
\end{tabular}
\end{table*}

==> contents/tables/weighted.tex <==
\begin{table}[]
\centering
\caption{Effect of weighted prototype estimation on the GTA $\rightarrow$ Cityscapes setting when using features from the mixed images for prototype estimation.}
\label{tab:weighted}
\begin{tabular}{@{}ccc@{}}
\toprule
Mixed Proto & Unweighted & Weighted      \\ \midrule
mIoU       & 60.1       & \textbf{62.2} \\ \bottomrule
\end{tabular}%
\end{table}
